Access Control Using Spatially Invariant Permutation of Feature Maps for Semantic Segmentation Models

In this paper, we propose an access control method that uses the spatially invariant permutation of feature maps with a secret key for protecting semantic segmentation models. Segmentation models are trained and tested by permuting selected feature maps with a secret key. The proposed method allows rightful users with the correct key not only to access a model to full capacity but also to degrade the performance for unauthorized users. Conventional access control methods have focused only on image classification tasks, and these methods have never been applied to semantic segmentation tasks. In an experiment, the protected models were demonstrated to allow rightful users to obtain almost the same performance as that of non-protected models but also to be robust against access by unauthorized users without a key. In addition, a conventional method with block-wise transformations was also verified to have degraded performance under semantic segmentation models.

==> sections/related.tex <==
Related Works.

\subsection{Semantic Segmentation}
The goal of semantic segmentation is to understand what is in an image at the pixel level.
Figure \ref{fig:semantic} shows an example of semantic segmentation.
The segmentation model takes an input image $x$ with the shape $c \times h \times w$ and outputs a segmentation map (SM) with the shape $1 \times h \times w$.
Here, $c$, $h$, and $w$ are the number of channels, height, and width of $x$, respectively, and each pixel in the SM represents a class label.
\begin{figure}[t]
	\centering
 	\centerline{\includegraphics[width=8.5cm] {./figures/semantic_segmentation.pdf}}
  	\caption{Example of semantic segmentation}
	\label{fig:semantic}
\end{figure}

One of the common metrics to evaluate segmentation performance is mean intersection-over-union (mean IoU) \cite{fcn, giou}, which first computes the IoU for each class and then computes the average over classes.
The IoU metric is the area of overlap between a predicted SM and a corresponding ground truth (GT) divided by the area of the union.
Mean IoU is defined as
\begin{equation}
    \mathrm{mean IoU}(SM, GT) = \frac{1}{class} \sum_{i=1}^{class} \frac{|SM_{i} \cap GT_{i}|}{|SM_{i} \cup GT_{i}|},
\end{equation}
where $class$ is the number of classes.
In addition, the metric ranges from zero to one, where a value of one means that a SM and a GT overlap perfectly, and a value of zero indicates no overlap.

\subsection{Model Protection}
Model Protection.

\subsection{Block-wise Transformation Protection}
Block-wise Transformation Protection.
